Computational Optimal Transport

Optimal transport (OT) theory can be informally described using the words of the French mathematician Gaspard Monge (1746-1818): A worker with a shovel in hand has to move a large pile of sand lying on a construction site. The goal of the worker is to erect with all that sand a target pile with a prescribed shape (for example, that of a giant sand castle). Naturally, the worker wishes to minimize her total effort, quantified for instance as the total distance or time spent carrying shovelfuls of sand. Mathematicians interested in OT cast that problem as that of comparing two probability distributions, two different piles of sand of the same volume. They consider all of the many possible ways to morph, transport or reshape the first pile into the second, and associate a "global" cost to every such transport, using the "local" consideration of how much it costs to move a grain of sand from one place to another. Recent years have witnessed the spread of OT in several fields, thanks to the emergence of approximate solvers that can scale to sizes and dimensions that are relevant to data sciences. Thanks to this newfound scalability, OT is being increasingly used to unlock various problems in imaging sciences (such as color or texture processing), computer vision and graphics (for shape manipulation) or machine learning (for regression, classification and density fitting). This short book reviews OT with a bias toward numerical methods and their applications in data sciences, and sheds lights on the theoretical properties of OT that make it particularly useful for some of these applications.

==> MAL-editorialboard.tex <==
\begin{editorialboard}

\subsection{Editor-in-Chief}

\journalchiefeditor{Michael Jordan}{University of California, Berkeley\\United States}



\subsection{Editors}
\begin{multicols*}{3}\raggedcolumns
\journaleditor{Peter Bartlett}{UC Berkeley}
\journaleditor{Yoshua Bengio}{Universit{\'e} de Montr{\'e}al}
\journaleditor{Avrim Blum}{CMU}
\journaleditor{Craig Boutilier}{University of Toronto}
\journaleditor{Stephen Boyd}{Stanford University}
\journaleditor{Carla Brodley}{Tufts University}
\journaleditor{Inderjit Dhillon}{Texas at Austin}
\journaleditor{Jerome Friedman}{Stanford University}
\journaleditor{Kenji Fukumizu}{ISM}
\journaleditor{Zoubin Ghahramani}{Cambridge University}
\journaleditor{David Heckerman}{Microsoft Research}
\journaleditor{Tom Heskes}{Radboud University}
\journaleditor{Geoffrey Hinton}{University of Toronto}
\journaleditor{Aapo Hyvarinen}{Helsinki IIT}
\journaleditor{Leslie Pack Kaelbling}{MIT}
\journaleditor{Michael Kearns}{UPenn}
\journaleditor{Daphne Koller}{Stanford University}
\journaleditor{John Lafferty}{University of Chicago}
\journaleditor{Michael Littman}{Brown University}
\journaleditor{Gabor Lugosi}{Pompeu Fabra}
\journaleditor{David Madigan}{Columbia University}
\journaleditor{Pascal Massart}{Universit{\'e} de Paris-Sud}
\journaleditor{Andrew McCallum}{University of Massachusetts Amherst}
\journaleditor{Marina Meila}{University of Washington}
\journaleditor{Andrew Moore}{CMU}
\journaleditor{John Platt}{Microsoft Research}
\journaleditor{Luc de Raedt}{Albert-Ludwigs-Universitaet Freiburg}
\journaleditor{Christian Robert}{Paris-Dauphine}
\journaleditor{Sunita Sarawagi}{IIT Bombay}
\journaleditor{Robert Schapire}{Princeton University}
\journaleditor{Bernhard Schoelkopf}{Max Planck Institute}
\journaleditor{Richard Sutton}{University of Alberta}
\journaleditor{Larry Wasserman}{CMU}
\journaleditor{Bin Yu}{UC Berkeley}
\end{multicols*}
\end{editorialboard} 

==> MAL-journaldata.tex <==
 \definecolor{palatinapurple}{rgb}{0.41, 0.16, 0.38}
\colorlet{MALcolor}{palatinapurple}   %new color names can be defined before use
\journalcolor      {MALcolor} %a color name.
\journaltitle      {Foundations and Trends\textsuperscript{\textregistered} in Machine Learning}
\journaltitleprefix{Foundations and Trends\textsuperscript{\textregistered} in}
\journalshorttitle {MAL}
\journalurl        {http://www.nowpublishers.com/MAL}
\journalissnprint  {1935-8237}
\journalissnonline {1935-8245}
\journaldoi        {10.1561/22}

\journalcopyrightowner{now Publishers Inc.}

\journalbibstyle{author} % either author or numeric

\journalaimsandscope
 {%
  Foundations and Trends\textsuperscript{\textregistered} in
Machine Learning publishes
 survey and tutorial articles in the following topics:
 \begin{multicols}{2}\raggedcolumns
 \begin{itemize}
\item{Adaptive control and signal processing}
\item{Applications and case studies}
\item{Behavioral, cognitive and neural learning}
\item{Bayesian learning}
\item{Classification and prediction}
\item{Clustering}
\item{Data mining}
\item{Dimensionality reduction}
\item{Evaluation}
\item{Game theoretic learning}
\item{Graphical models}
\item{Independent component analysis}
\item{Inductive logic programming}
\item{Kernel methods}
\item{Markov chain Monte Carlo}
\item{Model choice}
\item{Nonparametric methods}
\item{Online learning}
\item{Optimization}
\item{Reinforcement learning}
\item{Relational learning}
\item{Robustness}
\item{Spectral methods}
\item{Statistical learning theory}
\item{Variational inference}
\item{Visualization}
\end{itemize}
\end{multicols}
 }


\journallibraryinfo
 {%
  Foundations and Trends\textsuperscript{\textregistered} in
  Machine Learning, \useissuedata{pubyear},
  Volume~\useissuedata{volume}, 6 issues.
  ISSN paper version \usejournaldata{issnprint}.
  ISSN online version \usejournaldata{issnonline}.
  Also available as a combined paper and online
  subscription.
 } 

==> MAL-seriespage.tex <==
\vspace{12pt}
\noindent \textit{Non-convex Optimization for Machine Learningy}\\
Prateek Jain and Purushottam Ka\\
ISBN: 978-1-68083-368-3\\
\\
\noindent \textit{Kernel Mean Embedding of Distributions: A Review and Beyond}\\
Krikamol Muandet, Kenji Fukumizu, Bharath Sriperumbudur and\\ Bernhard Scholkopf\\
ISBN: 978-1-68083-288-4\\
\\
\noindent \textit{Tensor Networks for Dimensionality Reduction and Large-scale\\ Optimization: Part 1 Low-Rank Tensor Decompositions}\\
Andrzej Cichocki, Anh-Huy Phan, Qibin Zhao, Namgil Lee,\\ Ivan Oseledets, Masashi Sugiyama and Danilo P. Mandic\\
ISBN: 978-1-68083-222-8\\
\\
\noindent \textit{Tensor Networks for Dimensionality Reduction and Large-scale\\ Optimization: Part 2 Applications and Future Perspectives}\\
Andrzej Cichocki, Anh-Huy Phan, Qibin Zhao, Namgil Lee,\\ Ivan Oseledets, Masashi Sugiyama and Danilo P. Mandic\\
ISBN: 978-1-68083-276-1\\
\\
\noindent \textit{Patterns of Scalable Bayesian Inference}\\
Elaine Angelino, Matthew James Johnson and Ryan P. Adams \\
ISBN: 978-1-68083-218-1\\
\\
\noindent \textit{Generalized Low Rank Models}\\
Madeleine Udell, Corinne Horn, Reza Zadeh and Stephen Boyd \\
ISBN: 978-1-68083-140-5

==> NOWFnT-data.tex <==
\newcommand\nowfnt@publicationaddress
 {%
  \textit{Published, sold and distributed by:}\\
  now Publishers Inc.\\
  PO Box 1024\\
  Hanover, MA 02339\\
  United States\\
  Tel.\ +1-781-985-4510\\
  www.nowpublishers.com\\
  sales@nowpublishers.com%
  \par
  \textit{Outside North America:}\\
  now Publishers Inc.\\
  PO Box 179\\
  2600 AD Delft\\
  The Netherlands\\
  Tel.\ +31-6-51115274
 }

\newcommand\nowfnt@legalrightstext
 {%
  All rights reserved. No part of this publication may be
  reproduced, stored in a retrieval system, or transmitted in any form or by any means, mechanical, photocopying, recording or otherwise, without prior written permission of the publishers.
  \par
  Photocopying. In the USA: This journal is registered at the Copyright  Clearance Center, Inc., 222 Rosewood Drive, Danvers, MA 01923.  Authorization to photocopy items for
  internal or personal use, or the internal or personal use of specific  clients, is granted by now Publishers Inc for users registered with the Copyright Clearance Center (CCC).
  The `services' for users can be found on the internet at:
  www.copyright.com
  \par
  For those organizations that have been granted a photocopy license, a separate system of payment has been arranged. Authorization does not extend to other kinds of copying, such as that for general distribution, for advertising or promotional purposes, for creating new collective works, or for resale.  In the rest of the world:
  Permission to photocopy must be obtained from the copyright
  owner. Please apply to now Publishers Inc., PO Box 1024, Hanover, MA 02339, USA; Tel. +1 781 871 0245; www.nowpublishers.com; sales@nowpublishers.com
  \par
  now Publishers Inc. has an exclusive license to publish this
  material worldwide. Permission to use this content must be obtained from the copyright license holder. Please apply to now Publishers, PO Box 179, 2600
  AD Delft, The Netherlands, www.nowpublishers.com; e-mail:
  sales@nowpublishers.com}

\newcommand\nowfnt@printedoninfotext
 {%
  {%
   %
  }%
 }

\newcommand\nowfnt@howtocitetext
 {%
  The preferred citation for this publication is\par
  {%
   \raggedright
   \useissuedata{copyrightowner}.
   \emph{\nowfnt@articletitle}.
   \printjournaltitleprefix \usejournaldata{title}, vol.~\useissuedata{volume}, no.~\useissuedata{issue}, pp.~\useissuedata{firstpage}--\useissuedata{lastpage},
   \useissuedata{pubyear}.%
  }%
 }


\newcommand\nowfnt@copyrightlinetext
 {%
  ISBN: \useissuedata{isbn}\\
  \copyright\ \useissuedata{copyrightyear} \useissuedata{copyrightowner}}

\newcommand\nowfnt@NOWcopyrightlinetext  %for wrapper
  {%
  ISBN: \useissuedata{isbn}\\
  \copyright\ \useissuedata{copyrightyear} Now Publishers Inc}

\newcommand\nowfnt@sourceintro{%
 The content of the book was originally published in  }

\newcommand\nowfnt@sourcepunct{.}

\newcommand\nowfnt@prohibitiontext{}

\newcommand\nowfntstandardcitation{\nowfnt@authorlist@toc\ (\nowfnt@issuepubyear), \enquote{\nowfnt@articletitle}, \nowfnt@journaltitle: Vol. \nowfnt@issuevolume, No. \nowfnt@issueissue, pp \nowfnt@issuefirstpage--\nowfnt@issuelastpage. DOI: \nowfnt@issuedoi.}

%Title for the series pages.
\newcommand\nowfnt@seriespagetitle{\section*{Other titles in \nowfnt@journaltitle}}

==> frontmatter.tex <==
%% Front matter for for FnT Computer Graphics & Vision
%% (c) 2013 Neal Parikh (Stanford University)
%% 
%% Based on earlier NOW style files by S. Kumar,
%% J. Sebastian, T. Hoekwater, and B.V. Elvenkind

\RequirePackage{lastpage}
\RequirePackage{multicol}

% base journal information definitions
\def\doi#1{\def\@doi{#1}}
\def\copyrightowner#1{\def\@copyrightowner{#1}}
\def\firstpage#1{\def\@firstpage{#1}}
\def\isbn#1{\def\@isbn{#1}}
\def\issue#1{\def\@issue{#1}}
\def\journalinfofont{\fontsize{8}{10}\selectfont\rmfamily}
\def\journallibraryinfo#1{\def\@libraryinfo{#1}}
\def\journaltitle#1{\def\@journaltitle{#1}}
\def\journaltitleprefix#1{\def\@journaltitleprefix{#1}}
\def\@lastpage{\pageref{LastPage}}
\def\lastpage#1{\def\@lastpage{#1}}
\def\copyrightyear#1{\def\@copyrightyear{#1}}
\edef\@copyrightyear{\the\year}
\def\pubyear#1{\def\@pubyear{#1}}
\edef\@pubyear{\the\year}
\def\volume#1{\def\@volume{#1}}

\def\journaltopicintro#1{\def\@journaltopicintro{#1}}
\def\journaltopics#1{\def\@journaltopics{#1}}

% editors
\newcount\editorcount
\def\@editors{}
\def\journaleditor#1{%
  \advance\editorcount1 
  \ifx\empty\@editors
    \def\@editors{#1}%
  \else
    \expandafter\def\expandafter\@editors\expandafter{\@editors\\[0.3em]#1}%
  \fi
}

% editors in chief
\newcount\chiefeditorcount
\def\@chiefeditors{}
\def\journalchiefeditor#1{%
  \advance\chiefeditorcount1 
  \ifx\empty\@chiefeditors
    \def\@chiefeditors{#1}%
  \else
    \expandafter\def\expandafter\@chiefeditors\expandafter{\@chiefeditors\\[1em]#1}%
  \fi
}

%% title page

\renewcommand\maketitle{\begin{titlepage}%

\if@openright % -- for 'book' version
\parindent \z@

% title page
\thispagestyle{empty}
\vspace*{\fill}
\begin{flushright}
\begin{minipage}{0.8\textwidth}
\begin{flushright}
\renewcommand{\baselinestretch}{1.1}
\sffamily\bfseries\huge 
\@title
\end{flushright}
\end{minipage}
\end{flushright}
\vspace*{\fill}

% title+author page
\cleardoublepage
\thispagestyle{empty}

\begin{flushright}
{\renewcommand{\baselinestretch}{1.2}
\sffamily\Huge\bfseries \@title\par}
\vspace{3ex}
\noindent\rule{\textwidth}{2pt}
\vspace{1ex}\par

\begingroup
\def\and{%
  \end{tabular}%
  \par\vspace*{1.5ex}
  \begin{tabular}[t]{r@{}}
  \bfseries}

  \fontsize{13}{15}\selectfont\sffamily
\begin{tabular}[t]{r@{}}
    \bfseries
    \@author
\end{tabular}
\endgroup
\vfill
\includegraphics[width=53bp]{now_logo}\\
\includegraphics[width=81bp]{essence_logo}\\
Boston --- Delft
\end{flushright}

% publisher page
\newpage
\thispagestyle{empty}
\begingroup

\begin{minipage}{\textwidth}
\bfseries\sffamily\Large \@journaltitleprefix\\ \@journaltitle
\end{minipage}

\parskip6pt
\footnotesize

\vfill

{\itshape Published, sold and distributed by:}\\
now Publishers Inc.\\
PO Box 1024\\
Hanover, MA\ 02339\\
United States\\
Tel.\ +1-781-985-4510\\
www.nowpublishers.com\\
sales@nowpublishers.com

{\itshape Outside North America:}\\
now Publishers Inc.\\
PO Box 179\\
2600 AD Delft\\
The Netherlands\\
Tel.\ +31-6-51115274

The preferred citation for this publication is

{\raggedright
\@copyrightowner. \emph{\@title}.  \@journaltitleprefix\
\@journaltitle, vol.~\@volume, no.~\@issue, pp.~\@firstpage--\@lastpage,
\@pubyear.\par}

{\itshape This Foundations and Trends\textsuperscript{\textregistered} issue
was typeset in \LaTeX\ using a class file designed by Neal Parikh. Printed on
acid-free paper.}

ISBN: \@isbn\\ \copyright\ \@copyrightyear\ \@copyrightowner

\vfill

\fontsize{8}{9}\selectfont
All rights reserved. No part of this publication may be
reproduced, stored in a retrieval system, or transmitted in any form
or by any means, mechanical, photocopying, recording or otherwise,
without prior written permission of the publishers.

Photocopying. In the USA: This journal is registered at the Copyright
Clearance Center, Inc., 222 Rosewood Drive, Danvers, MA 01923. 
Authorization to photocopy items for
internal or personal use, or the internal or personal use of specific
clients, is granted by now Publishers Inc for users registered with 
the Copyright Clearance Center (CCC).
The `services' for users can be found on the internet at:
www.copyright.com

For those organizations that have been granted a photocopy license, a
separate system of payment has been arranged. Authorization does not
extend to other kinds of copying, such as that for general
distribution, for advertising or promotional purposes, for creating
new collective works, or for resale.  In the rest of the world:
Permission to photocopy must be obtained from the copyright
owner. Please apply to now Publishers Inc., PO Box 1024, Hanover, MA
02339, USA; Tel. +1 781 871 0245; www.nowpublishers.com;
sales@nowpublishers.com

now Publishers Inc. has an exclusive license to publish this
material worldwide. Permission to use this content must be obtained from
the copyright license holder. Please apply to now Publishers, PO Box 179, 2600
AD Delft, The Netherlands, www.nowpublishers.com; e-mail:
sales@nowpublishers.com\par
\endgroup

% editorial board
\newpage
\thispagestyle{empty}
\begin{center}
\sffamily\LARGE
{\bfseries \@journaltitleprefix\\ \@journaltitle}\\
{Volume \@volume, Issue \@issue, \@pubyear}\\
{\bfseries Editorial Board}
\end{center}

\vspace{8pt}

\ifnum\chiefeditorcount>1
{\sffamily\bfseries Editors-in-Chief}
{\footnotesize
\begin{multicols}{2}
\@chiefeditors
\end{multicols}}
\else
{\sffamily\bfseries Editor-in-Chief}\par
\vspace*{10pt}
\begin{footnotesize}
\begin{tabular}[t]{@{}l}
\@chiefeditors \\
\end{tabular}
\end{footnotesize}
\vspace*{10pt}
\fi

{\sffamily \bfseries Editors}
{\fontsize{9}{11}\selectfont
\begin{multicols}{3}
\raggedcolumns
\@editors
\end{multicols}}%

% editorial scope
\newpage % page vi -- blank
\thispagestyle{empty}
\begin{center}
{\sffamily\bfseries\LARGE Editorial Scope}
\end{center}

\vspace{18pt}

{\bfseries\large\sffamily Topics}\\

\@journaltopicintro\par

\fontsize{10}{13}\selectfont
\begin{multicols}{2}
    \raggedright
    \@journaltopics
\end{multicols}

{\bfseries\large\sffamily Information for Librarians}\\

\@libraryinfo\par

\else\fi % -- no book front matter for "journal" version

% -- end book front matter

% title+author page
\newpage
\thispagestyle{empty}
\hbox to \textwidth{%
%% modified GP
\if 0
    \vbox{\raggedright
    \hsize=.6\textwidth \journalinfofont
{\hangindent=3.5ex
\hangafter=1
\@journaltitleprefix\\ \@journaltitle\par}%
Vol.~\@volume, No.~\@issue\ (\@pubyear) 
\@firstpage--\@lastpage\\
{\hangindent=3.5ex
\hangafter=1
\copyright\ \@copyrightyear\ \@copyrightowner\par}%
DOI: \@doi}\hss
\vbox{\hsize=.4\textwidth 
    \raggedleft
    \includegraphics[width=53bp]{now_logo}\\
    \includegraphics[width=81bp]{essence_logo}\\
    \par
} %
\fi
%%% GP
}\par
\let\footnoterule\relax
\let\footnote\thanks
\null\vfil
\vskip 60\p@
\begin{center}%
{\LARGE \sffamily \bfseries \@title \par}%
\vskip 3em%
{
\large
\lineskip .75em%
     \lineskip .75em%
      \begin{tabular}[t]{c}%
        \@author
      \end{tabular}\par}%
\end{center}\par
\@thanks
\vfill
\end{titlepage}
\setcounter{footnote}{0}%
}

%% defaults and settings for this FnT

\def\@copyrightowner{now Publishers Inc.}
\journaltitleprefix{Foundations and Trends\textsuperscript{\textregistered} in}
\volume{XX}
\issue{XX}
\firstpage{1}
\isbn{XXX-X-XXXXX-XXX-X}
\doi{10.1561/XXXXXXXXXX}

\journaltitle{Computer Graphics and Vision}

\journalchiefeditor{\textbf{Brian Curless} \\
University of Washington \\
United States}

\journalchiefeditor{\textbf{William T. Freeman}\\
Massachusetts Institute of Technology \\
United States \columnbreak}

\journalchiefeditor{\textbf{Luc Van Gool} \\
KU Leuven, Belgium \\
ETH Zurich, Switzerland \columnbreak}


\journaleditor{Marc Alexa \\ \emph{TU Berlin}}
\journaleditor{Ronen Basri \\ \emph{Weizmann Institute}}
\journaleditor{Peter Belhumeur \\ \emph{Columbia University}}
\journaleditor{Andrew Blake \\ \emph{Microsoft Research}}
\journaleditor{Chris Bregler \\ \emph{New York University}}
\journaleditor{Joachim Buhmann \\ \emph{ETH Zurich}}
\journaleditor{Michael Cohen \\ \emph{Microsoft Research}}
\journaleditor{Paul Debevec \\ \emph{USC ICT}}
\journaleditor{Julie Dorsey \\ \emph{Yale University}}
\journaleditor{Fredo Durand \\ \emph{MIT}}
\journaleditor{Olivier Faugeras \\ \emph{INRIA}}
\journaleditor{Mike Gleicher \\ \emph{University of Wisconsin}\columnbreak}
\journaleditor{Richard Hartley \\ \emph{ANU}}
\journaleditor{Aaron Hertzmann \\ \emph{University of Toronto}}
\journaleditor{Hugues Hoppe \\ \emph{Microsoft Research}}
\journaleditor{C. Karen Liu \\ \emph{Georgia Tech}}
\journaleditor{David Lowe \\ \emph{UBC}}
\journaleditor{Jitendra Malik \\ \emph{UC Berkeley}}
\journaleditor{Steve Marschner \\ \emph{Cornell University}}
\journaleditor{Shree Nayar \\ \emph{Columbia University}}
\journaleditor{James O'Brien \\ \emph{UC Berkeley}}
\journaleditor{Tomas Pajdla \\ \emph{Czech TU}}
\journaleditor{Pietro Perona \\ \emph{Caltech}}
\journaleditor{Marc Pollefeys \\ \emph{ETH Zurich}\columnbreak}
\journaleditor{Jean Ponce \\ \emph{UIUC}}
\journaleditor{Long Quan \\ \emph{HKUST}}
\journaleditor{Cordelia Schmid \\ \emph{INRIA}}
\journaleditor{Steve Seitz \\ \emph{University of Washington}}
\journaleditor{Amnon Shashua \\ \emph{Hebrew University}}
\journaleditor{Peter Shirley \\ \emph{University of Utah}}
\journaleditor{Stefano Soatto \\ \emph{UCLA}}
\journaleditor{Richard Szeliski \\ \emph{Microsoft Research}}
\journaleditor{Joachim Weickert \\ \emph{Saarland University}}
\journaleditor{Song Chun Zhu \\ \emph{UCLA}}
\journaleditor{Andrew Zisserman \\ \emph{University of Oxford}}

\journaltopicintro{\@journaltitleprefix\ \@journaltitle\ publishes
survey and tutorial articles in the following topics:}

\journaltopics{
\begin{itemize}\itemsep=0pt
    \item{Rendering}
    \item{Shape}
    \item{Mesh simplification}
    \item{Animation}
    \item{Sensors and sensing}
    \item{Image restoration and enhancement}
    \item{Segmentation and grouping}
    \item{Feature detection and selection}
    \item{Color processing}
    \item{Texture analysis and synthesis}
    \item{Illumination and reflectance modeling}
    \item{Shape representation}
    \item{Tracking}
    \item{Calibration}
    \item{Structure from motion}
    \item{Motion estimation and registration}
    \item{Stereo matching and reconstruction}
    \item{3D reconstruction and image-based modeling}
    \item{Learning and statistical methods}
    \item{Appearance-based matching}
    \item{Object and scene recognition}
    \item{Face detection and recognition}
    \item{Activity and gesture recognition}
    \item{Image and video retrieval}
    \item{Video analysis and event recognition}
    \item{Medical image analysis}
    \item{Robot localization and navigation}
\end{itemize}
}

\journallibraryinfo{%
  Foundations and Trends\textsuperscript{\textregistered} in \@journaltitle, \@pubyear,
  Volume~\@volume, 4 issues. ISSN paper version 1572-2740. %%% (\@paperprice).
  ISSN online version 1572-2759. %%% (\@onlineprice).
  Also available as a combined paper and online
  subscription.%%% (\@combinedprice).
}

\endinput

